Assessing the Linguistic Quality of REST APIs for IoT Applications

Internet of Things (IoT) is a growing technology that relies on connected 'things' that gather data from peer devices and send data to servers via APIs (Application Programming Interfaces). The design quality of those APIs has a direct impact on their understandability and reusability. This study focuses on the linguistic design quality of REST APIs for IoT applications and assesses their linguistic quality by performing the detection of linguistic patterns and antipatterns in REST APIs for IoT applications. Linguistic antipatterns are considered poor practices in the naming, documentation, and choice of identifiers. In contrast, linguistic patterns represent best practices to APIs design. The linguistic patterns and their corresponding antipatterns are hence contrasting pairs. We propose the SARAv2 (Semantic Analysis of REST APIs version two) approach to perform syntactic and semantic analyses of REST APIs for IoT applications. Based on the SARAv2 approach, we develop the REST-Ling tool and empirically validate the detection results of nine linguistic antipatterns. We analyse 19 REST APIs for IoT applications. Our detection results show that the linguistic antipatterns are prevalent and the REST-Ling tool can detect linguistic patterns and antipatterns in REST APIs for IoT applications with an average accuracy of over 80%. Moreover, the tool performs the detection of linguistic antipatterns on average in the order of seconds, i.e., 8.396 seconds. We found that APIs generally follow good linguistic practices, although the prevalence of poor practices exists.

==> CoverLetter.tex <==
\section*{COVER LETTER}

We thank the reviewers for their insightful feedback. We have taken all the comments seriously and made our effort to revise the manuscript. We also made a thorough proof read to improve the readability of the manuscript. 

The major changes in the revised manuscript include:

\begin{itemize}
    \item We made a new validation with the same 91 URIs, but this time for each of the 9 antipattens, thus, in total 819 questions were asked for each manual validation;
    \item We revised Section 2 on how we actually defined new linguistic antipatterns;
    \item We revisited Section 3 to cut down parts that are not essential to understand the study, thus, shorted and removed some texts and figures that can be found in our previous/related studies;
    \item We re-organized the Sections according to the suggestions from the reviews;
    \item We added a new research question on Efficiency of the tool, thus, we have four research question now;
    \item We modified our results tables to have a horizontal view and to be consistent with relevant figures in terms of visualization;
    \item We revised our Validation Process Section and introduced the MCC and Accuracy as our new measure instead of Precision/Recall;
    \item We re-ordered the research questions to have a better flow of the study and results;
\end{itemize}

Some minor changes include:

\begin{itemize}
    \item We revised the Abstract to fit our new version of the manuscript;
    \item We also revised part of our Introduction to reflect our revised manuscript, e.g., added the new research question and updated the contribution part;

    \item We modified the Conclusion Section to reflect our revised manuscript;
    \item We made a thorough proof read of the manuscript;
    \item We provided the new validation dataset online \url{https://doi.org/10.5281/zenodo.6393404}.
\end{itemize}

==> JSSReview2-2021.tex <==
\input{CoverLetter}

\input{Responses}

==> Responses.tex <==
\section*{Response to the Feedback:}

\noindent\textbf{Reviewer \#2:} My main concern for the original submission was the contributions of the current article with respect to previous work for the authors. In the revised version, the authors more precisely identified the added contributions of the current article. The contributions are still incremental, but I feel that performing the experiments on the 19 APIs, analyzing them with respect to the linguistic patterns, and developing the REST-Ling tool, could be useful for other researchers.

\noindent\textbf{Response:} We thank the reviewer for the encouraging remark. We believe our study is one of the very few that focused on the linguistic design quality of the APIs. Thus, we hope developers community and researchers would benefit from our study.\newline\newline

\noindent\textbf{R2.2 and R2.3:} the change of SANTA to SARAv2 clarifies the difference. However, I still recommend the following minor adjustments (as far as I understood the paper).

- SARAv2 is an approach to perform syntactic and semantic analyses of REST APIs. (Instead of IoT APIs, as there is no IoT-specific new or existing pattern). This could be changed in the abstract.

- Page 3, contributions, contribution 1: clarify that SARAv2 is an extension of existing SARA by 3 new patterns (are there any significant extensions with respect to SARAv1?)

- The patterns of SARAv2 and the REST-Ling tool is used in the current paper for IoT APIs. This is correctly described in the contributions.

- In the related work: "Firstly, our SARAv2 approach is the first attempt in studying the APIs from IoT providers" - rephrase, because SARAv2 is a general approach for analyzing REST APIs, and the empirical experiment in the current paper is the first study related to IoT APIs.

- In the conclusion, the difference is more clearly defined ("We proposed the SARAv2 approach and used it to perform syntactic and semantic analyses of REST APIs for IoT applications")

\noindent\textbf{Response:} Thank you for the various comments above. We have taken care to revise our manuscript based on the above suggestions in various places and we thank the reviewer for these suggestions.\newline\newline

\noindent\textbf{R2.2:} I still feel that much of Section 3 is not necessarily needed in the current paper. The patterns are defined in Section 2. In Section 3 the high-level overview is relevant from the point of view of the current paper: the SOFA framework is used to detect these patterns, but how these patterns are exactly detected is prior work that is currently reused. Nevertheless, I see how it makes the paper more self-contained, but it becomes unnecessarily longer than needed and is harder to focus on the new contribution.

\noindent\textbf{Response:} We agree with the reviewer in the fact that keeping some parts of Section 3 is repetitive and makes the manuscript longer. We removed some parts from Section 3 that are not required to understand our approach. However, we chose to keep the example on how compare two URIs in order to perform semantic similarity between them, which will make the manuscript self-contained.\newline\newline

\noindent\textbf{R2.4:} The paper still says, "using the random sampling we randomly chose 90 URIs (thus, 90 questions) out of 1,102 URIs from 19 APIs to measure the overall precision." But only one pattern was checked for each URI, and it is not mentioned, how and which pattern was chosen for each API. As far as I can see from the dataset, the distribution of the patterns+antipatterns are not uniform (e.g., URI versioning + Unversioned URI = 5, while Consistent + Inconsistent documentation = 20). It seems that the questions (a question is a URI + pattern/antipattern detection) were randomly chosen. But then the population size is 9 * 1102 and not 1102. Note: I'm not asking to increase the sample size; just adjust the reported confidence level and explain the selection procedure.

\noindent\textbf{Response:} We agree with this comment. We also received a similar comment from the other review. Now, based on the comments from the other reviewer, we made a new validation on a larger sample. Plus, the distribution of the patterns and antipatterns are now uniform. More specifically, previously we only selected 90 URIs randomly regardless of the detection of patterns and antipatterns on them. Thus, previously we had 91 questions in total to ask each validator. Now, with the new validation plan, we have 91 URIs and they are validated for all antipatterns, i.e., 91 x 9 = 819 questions in total to ask for each validator. We also have updated the Validation Process section accordingly.\newline\newline

\noindent\textbf{R2.6:} I think Table 5 still calculates averages for the two sides of the same binary classification. There is an average row at the bottom, which is the average of all the above rows. But for example, Amorphous URI and Tidy URI are not two separate detection rules; they are the positive and negative results of the same rule. I'm not an expert in statistics but calculating the average of these two rows for precision seems to be problematic for me. I would recommend having one row for each rule, and having four columns (TP, FP, FN, TN) to help calculate the full confusion matrix. Calculate Matthews correlation coefficient (MCC) additionally to precision and recall. MCC is a better metric because it "is invariant if the positive class is renamed negative and vice versa" [2]. Therefore, it results in the same value if a row displays the pattern or the antipattern (which generally flips the confusion matrix). Moreover, MCC takes into account all four values in the confusion
matrix to provide an overall metric about the performance.

\noindent\textbf{Response:} We agree with the reviewer and we would like to thank the reviewer for the suggestions. We agree that the calculated average values were not representative. We have now revised the validation table with new validation dataset. Because we now validated for all antipatterns for the sampled URIs we are now able to calculate the confusion matrix, and thus, the MCC and accuracy value, as shown in the table.\newline\newline

\noindent\textbf{Other Issues:}

- The structure of Section 4 is a bit odd. Now it is Subjects and Objects (4.1), Overview of results (4.2), RQs (4.3), Process (4.4), RQ1 details (4.5), RQ2 details, RQ3 details, Efficiency of REST-Ling, Presenting REST-Ling tool (4.9), Threats to validity.

  - The first paragraph of Section 4 talks about two studies, but it was not evident to me, which are the two studies and which RQ belongs to which study.
  
  - Moreover, some results are presented in 4.1, while similar ones are in 4.5.
  
  - I recommend restructuring this section according to common guidelines for reporting SE experiments (e.g. [1]). For example:  Goal/RQ, Subjects and objects, Process (add the general process also and not just validation), Results for RQs (each RQ a subsection), Threats to validity.
  
  - Efficiency of REST-Ling could be a separate RQ (as it also provides empirical evidence). In my opinion, "Operationalising REST-Ling Tool" is about presenting the REST-Ling tool. As such, it could go into Section 3, where the approach is introduced (it is not about the empirical results).
  
  - The RQs can be reordered: current RQ1 and RQ3 are about the APIs, while RQ2 and the efficiency of REST-Ling are about validating the accuracy and runtime performance of the tool and the approach. These two aspects are now not separated, but they should be separated. For example, RQ1.1 <- current RQ1 and RQ1.2 <- current RQ3 (what we discovered about IoT APIs) and RQ2.1 <- current RQ2 and RQ2.2 <- efficiency (are the previous results valid)?

\noindent\textbf{Response:} We thank the reviewer for the detailed suggestions. We agree with the comments and we have taken into account all the suggestions offered. In particular, we have restructured the sections to fit common guidelines for SE experiments. We also introduced a new RQ on efficiency. We have moved the section on "Operationalising REST-Ling Tool" together with the Approach section. We also have reordered the RQs as suggested by the reviewer to improve the flow. We believe this helped us having with a coherent flow.\newline\newline

\textbf{Minor comments:}

- abstract: "we develop the REST-Ling tool and empirically validate for the detection results of nine linguistic antipatterns." -> I would remove "for"

- intro: "to the best API design practice" -> maybe use good instead of best (in my opinion, good practices is a better phrase than best practices)

- Figure 6 and Table 4 presents the same data, but the orientation of Table 4 makes it a bit hard to compare them. In Figure 6, pattern names are on the top and IoT APIs are listed top to bottom. Table 4 is transposed. Instead of having a rotated landscape-oriented table, could not the data fit into a portrait table with rotated pattern names in the top and APIs in rows in the same order as Figure 6?

- "We involved three professionals" it can be clarified here that two of them were co-authors of the paper (Tobies, Havier) and the third one an external professional.

- Section 4.5, page 23: "In Table 6, the first column shows" --- isn't it Table 4?

[1] Jedlitschka A., Ciolkowski M., Pfahl D. (2008) Reporting Experiments in Software Engineering. In: Shull F., Singer J., Sjøberg D.I.K. (eds) Guide to Advanced Empirical Software Engineering. Springer, London. https://doi.org/10.1007/978-1-84800-044-5\_8

[2] Chicco, D., \& Jurman, G. (2020). The advantages of the Matthews correlation coefficient (MCC) over F1 score and accuracy in binary classification evaluation. BMC genomics, 21(1), 6. https://doi.org/10.1186/s12864-019-6413-7

\noindent\textbf{Response:} We thank the reviewer for identifying these issues. We have revised them in the manuscript. In particular, we have the mosaic plot and the corresponding results table coherent. We also fixed other minor typos.\newline\newline

\noindent\textbf{Reviewer \#3:} Thank you for putting considerable effort into addressing these review comments. Unfortunately, it does not seem that all of the comments are appropriately dealt with.

\noindent\textbf{R1-1.} The authors did not clearly answer this question. How was the simplistic form of the grounded theory approach conducted? Please elaborate on this.  Specifically, it should be shown how many inspectors join, and how to deal with conflicts. The process should be designed in order to remove bias by specific inspectors.

\noindent\textbf{Response:} Our apologies for not properly clarifying our approach. We have now revised the manuscript with proper clarification. 

Indeed, we should not have claimed to follow a (simplistic) grounded theory approach to define the new antipatterns and patterns. We carried out an analysis of the literature, followed by a data analysis, by also looking at the URIs and API documentation in our API dataset, we create "themes" of patterns and antipatterns that are applicable to REST URIs and documentation, by using thematic analysis based on the method proposed by Braun, Virginia, and Victoria Clarke. "Using thematic analysis in psychology." Qualitative research in psychology 3.2 (2006): 77-101. However we did not apply an iterative and thorough approach, as in Fully-fledged Grounded Theory. Hence, it would be unfair to claim that "we followed a ground theory approach". Thus, in the manuscript, we revisited our process of defining new linguistic antipatterns.\newline\newline


%\textcolor{blue}
%{Of course we cannot claim the list of linguistic patterns and anti-patterns
%is complete, there URIs or documentation that we are not considering, and,
%other type of linguistic patterns and antipatterns might be defined, using different Natural-Language Processing techniques. Therefore when talking about linguistic quality of IoT APIs, we do it based on the set of patterns and antipatterns on our approach. Nevertheless, at the best of our knowledge, our approach and the empirical study performed on RESTFul IoT APIs is the widest and deepest analysis so far. This limitation has been also introduced in the Threats to the Validity section}

\noindent\textbf{R1-2.} Regarding Table 7, it is unclear whether the authors applied the previous methods to the dataset used in this study. This should be the case in order to ensure a fair comparison. If not, and a fair comparison is impossible, this should be clarified and the reason given.

\noindent\textbf{Response:} We agree with the reviewer and we would like to thank the reviewer for the feedback. Originally, it was not our intention to apply previous methods to our dataset in this study. Indeed, it would not be a fair to compare the detection accuracy of different methods that are tailored to different datasets. Although a partial comparison is possible with SARA and CloudLex approach, that would not give a complete picture. Moreover, the CloudLex method performed detection for only two linguistic antipatterns from the list of our linguistic antipatterns in this manuscript. Thus, we slightly modified our 2nd research question to compare only the prevalence of linguistic antipatterns, and discarded the unfair and partial comparison of detection accuracy. However, as we made a general comparison of the studies in the literature in the Related Work section, we also showed a overall comparison of the studies from accuracy/precision viewpoint without being judgmental. We believe sort of partial comparison is suitable in the Related Work section. Please note that the comparison we made in RQ2 (on Comparison) concerns the prevalence of linguistic antipatterns across domain, instead of the accuracy of the methods that exist in the literature.\newline\newline

\noindent\textbf{R1-4.} The problem is the approach to sampling, and not the sample size itself. Using APIs from one project makes the results biased. Thus, the authors should conduct random sampling with a confidence level of 95\% and a confidence interval of 10 at the most. (Actually, this interval is a bit lax, and 5 would be better.) That is, 90 URIs (i.e., 810 questions) should be inspected. This number is realistic enough, and this approach would simplify the validation. 

\noindent\textbf{Response:} We thank the reviewer for the suggestion. We now performed a new validation with a new dataset. We considered a confidence level of 95\% and confidence interval of 10, thus, we got 91 URIs to validated and with 9 antipatterns, we had a total of 819 questions to ask for each validator. Please refer to R2.4 above that also referred to the same problem in our validation, and that we fixed now in the new version of the manuscript.\newline\newline

\noindent\textbf{R1-12.} The authors did not answer the question about the performance. Does the proposed method outperform the previous methods and should developers always use the proposed methods? Also, this question should be answered: "what is the conclusion and what is the message that the reader should get?"

\noindent\textbf{Response:} We thank the reviewer for the comment. Please refer to R1-2 above. We have now slightly modified our RQ2 (on Comparison) and now moved the partial comparison of the accuracy to the Related Work section for an overall, partial comparison. We believe it would not be fair to make a partial comparison among the various methods to analyse APIs in different domains, and trying to answer RQ2 on partial observation. However, we now moved the accuracy comparison table to the Related Work section for providing a synopsis.\newline\newline

\noindent\textbf{Minors:}
The contributions and abstract should be updated to include the result of RQ3.

The title of Section 4.6 is wrong. It should be "RQ2 Accuracy: " instead of "RQ2 Comparison: "

In Section 3.3.5, the phrase "by Mohaet al. [30]." needs a space between "Maha" and "et al."

\noindent\textbf{Response:} We thank the reviewer for noticing these. We have revised them in the manuscript accordingly.\newline\newline

==> makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> oldRQ2.tex <==
\subsection{\textbf{RQ$_2$ Proneness: Do IoT APIs generally follow poor design practices as opposed to the good design practices, or vice versa?}}

In RQ$_1$, we showed the prevalence of linguistic antipatterns in IoT APIs in terms of total detected instances. Here, we want to analyze, through a series a statistical tests, whether IoT APIs in general follow poor linguistic design practices. Our assumption is that, for each IoT API, there is no difference between the total number of instances for linguistic antipatterns and the total number of instances for linguistic patterns, \textit{i.e.}, the \textit{null} hypothesis.

\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.33\textwidth]{images/01AmorTidy.pdf}
\hfill
\includegraphics[width=0.33\textwidth]{images/02Context.pdf}
\hfill
\includegraphics[width=0.33\textwidth]{images/03CRUD.pdf}
\caption{Comparison of Amorphous URI \textit{vs.} Tidy URI (left), Contextless Resource Names \textit{vs.} Contextualised Resource Names (middle), and CRUDy URI \textit{vs.} Verbless URI (right) instances in 19 APIs.} \label{fig:comp01}
\end{center}
\end{figure}

\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.33\textwidth]{images/04Hier.pdf}
\hfill
\includegraphics[width=0.33\textwidth]{images/05Plu.pdf}
\hfill
\includegraphics[width=0.33\textwidth]{images/06Pert.pdf}
\caption{Comparison of Non-Hierarchical Nodes \textit{vs.} Hierarchical Nodes (left), Pluralised Nodes \textit{vs.} Singularised Nodes (middle), and Non-pertinent Documentation \textit{vs.} Pertinent Documentation (right) instances in 19 APIs.} \label{fig:comp02}
\end{center}
\end{figure}

\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.33\textwidth]{images/07Inconsistent.pdf}
\hfill
\includegraphics[width=0.33\textwidth]{images/08Version.pdf}
\hfill
\includegraphics[width=0.33\textwidth]{images/09Standard.pdf}
\caption{Comparison of Inconsistent Documentation \textit{vs.} Consistent Documentation (left), Unversioned URI \textit{vs.} URI Versioning (middle), and Non-standard URI \textit{vs.} Standard URI (right) instances in 19 APIs.} \label{fig:comp03}
\end{center}
\end{figure}

\begin{table}[t!]
    \centering
    \footnotesize
    \begin{tabular}{l|c|c}
\toprule
Treatment Groups & Treatment Type & p-value \\
\midrule
Amorphous URI $\sim$ Tidy URI &  & 0.00014 \\
Contextless Resource Names $\sim$ Contextualised Resource Names &  & 0.00014 \\
CRUDy URI $\sim$ Verbless URI &  & 0.00014 \\
Non-Hierarchical Nodes $\sim$ Hierarchical Nodes &  & 0.00014 \\
Pluralised Nodes $\sim$ Singularised Nodes & Number of Instances Detected in 19 APIs & 0.00072 \\
Non-pertinent Documentation $\sim$ Pertinent Documentation &  & 0.27572 \\
Inconsistent Documentation $\sim$ Consistent Documentation &  & 0.00014 \\
Unversioned URI $\sim$ URI Versioning &  & 0.11642 \\
Non-standard URI $\sim$ Standard URI &  & 0.00016 \\
\bottomrule
    \end{tabular}
    \caption{The Wilcoxon Rank Sum Test between Antipattern and Pattern Instances for 19 APIs.}
    \label{tab:test01}
\end{table}

\begin{table}[t!]
    \centering
    \footnotesize
    \begin{tabular}{l|c|c}
\toprule
Treatment Groups & Treatment Type & Cliff's $\delta$ \\
\midrule
Amorphous URI $\sim$ Tidy URI &  & -0.9833795 (large) \\
Contextless Resource Names $\sim$ Contextualised Resource Names &  & -0.8975069 (large) \\
CRUDy URI $\sim$ Verbless URI &  & -0.9833795 (large) \\
Non-Hierarchical Nodes $\sim$ Hierarchical Nodes &  & -1 (large) \\
Pluralised Nodes $\sim$ Singularised Nodes & Number of Instances Detected in 19 APIs & -0.4903047 (large) \\
Non-pertinent Documentation $\sim$ Pertinent Documentation &  & 0.1024931 (negligible) \\
Inconsistent Documentation $\sim$ Consistent Documentation &  & -0.8947368 (large) \\
Unversioned URI $\sim$ URI Versioning &  & 0.3518006 (medium) \\
Non-standard URI $\sim$ Standard URI &  & -0.9916898 (large) \\
\bottomrule
    \end{tabular}
    \caption{The Wilcoxon Rank Sum Test between Antipattern and Pattern Instances for 19 APIs.}
    \label{tab:test02}
\end{table}

To test the null hypothesis, we use the two-tailed Wilcoxon rank sum test and investigate whether IoT APIs have more antipattern instances than the instances of pattern, or vice versa. For a comparison that exhibits a statistically significant difference, we also compute the Cliff’s $\delta$ effect size \cite{kelley2012effect} to quantify the magnitude of the difference. We perform all the tests using the 5\% significance level (\textit{i.e.}, \textit{p-value<0.05}). The magnitude is assessed using these thresholds: if $\delta$<0.147 then \textit{negligible}, else if $\delta$<0.33 then \textit{small}. When the $\delta$<0.474 then it is \textit{medium}, otherwise the magnitude is \textit{large}.

The significant portion of the tested URIs follow \textit{Tidy URI}, \textit{Contextualised Resource Names}, and \textit{Verbless URI} patterns as opposed to their corresponding antipatterns \textit{Amorphous URI}, \textit{Contextless Resource Names}, and \textit{CRUDy URI} (see Figure \ref{fig:comp01}). Moreover, we also observed an indication that \textit{Hierarchical Nodes} and \textit{Singularised Nodes} patterns are more common than their corresponding antipatterns \textit{Non-Hierarchical Nodes} and \textit{Pluralised Nodes} in the IoT APIs (see Figure \ref{fig:comp02}). However, as shown in Figure \ref{fig:comp02}, APIs are found to have higher number of \textit{Non-pertinent Documentation} antipattern (i.e., more than 60\% cases) than its corresponding pattern. Finally, seen in Figure \ref{fig:comp01}, we observe that developers usually write consistent documentation and design standard URIs for their URIs, i.e., very few instances of \textit{Inconsistent Documentation} and \textit{Non-standard URI} antipatterns. Although, we also found that API developers often do not include version info in their URI design choices.

Our findings are confirmed using the wilcoxon rank sum test in Table \ref{tab:test01}. In summary, the \textit{Tidy URI}, \textit{Contextualised Resource Names}, \textit{Verbless URI}, \textit{Hierarchical Nodes}, \textit{Singularised Nodes}, and \textit{Standard URI} linguistic design patterns are found more than their corresponding linguistic antipatterns at the statistically significant level. Although the \textit{Non-pertinent Documentation} and \textit{Unversioned URI} antipatterns are more common than their corresponding \textit{Pertinent Documentation} and \textit{URI Versioning} patterns, these are not statistically significant. The results are further confirmed using Cliff’s $\delta$, as shown in Table \ref{tab:test02}.

\begin{center}
\begin{tcolorbox}[colback=gray!15,%gray background
                  colframe=gray,% black frame colour
                  width=12cm,% Use 5cm total width,
                  left=1pt,
                  right=1pt,
                  top=1pt,
                  bottom=1pt,
                  arc=1mm, auto outer arc]
\textbf{Summary on RQ$_2$ Proneness:} As concluded in RQ$_{1}$, linguistic antipatterns are prevalent in IoT APIs. However, further statistical tests confirmed that \textbf{linguistic design patterns are more common than linguistic antipatterns except for two cases (\textit{Non-pertinent Documentation} and \textit{Unversioned URI})}. This suggests that API developers are well aware of good API design practices. Although all the analysed IoT APIs are found to have between two and six different linguistic antipatterns.  
\end{tcolorbox}
\end{center}
